VIENA2: A Driving Anticipation Dataset

Action anticipation is critical in scenarios where one needs to react before the action is finalized. This is, for instance, the case in automated driving, where a car needs to, e.g., avoid hitting pedestrians and respect traffic lights. While solutions have been proposed to tackle subsets of the driving anticipation tasks, by making use of diverse, task-specific sensors, there is no single dataset or framework that addresses them all in a consistent manner. In this paper, we therefore introduce a new, large-scale dataset, called VIENA2, covering 5 generic driving scenarios, with a total of 25 distinct action classes. It contains more than 15K full HD, 5s long videos acquired in various driving conditions, weathers, daytimes and environments, complemented with a common and realistic set of sensor measurements. This amounts to more than 2.25M frames, each annotated with an action label, corresponding to 600 samples per action class. We discuss our data acquisition strategy and the statistics of our dataset, and benchmark state-of-the-art action anticipation techniques, including a new multi-modal LSTM architecture with an effective loss function for action anticipation in driving scenarios.

==> 0353 <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\providecommand{\doi}[1]{https://doi.org/#1}

\bibitem{aliakbarian2017encouraging}
Aliakbarian, M.S., Saleh, F.S., Salzmann, M., Fernando, B., Petersson, L.,
  Andersson, L.: Encouraging lstms to anticipate actions very early. In: ICCV
  (2017)

\bibitem{DynamicNetwork}
Bilen, H., Fernando, B., Gavves, E., Vedaldi, A., Gould, S.: Dynamic image
  networks for action recognition. In: CVPR (2016)

\bibitem{chan2016anticipating}
Chan, F.H., Chen, Y.T., Xiang, Y., Sun, M.: Anticipating accidents in dashcam
  videos. In: ACCV (2016)

\bibitem{LRCN}
Donahue, J., Anne~Hendricks, L., Guadarrama, S., Rohrbach, M., Venugopalan, S.,
  Saenko, K., Darrell, T.: Long-term recurrent convolutional networks for
  visual recognition and description. In: CVPR (2015)

\bibitem{dong2017intention}
Dong, C., Dolan, J.M., Litkouhi, B.: Intention estimation for ramp merging
  control in autonomous driving. In: IV (2017)

\bibitem{feichtenhofer2017spatiotemporal}
Feichtenhofer, C., Pinz, A., Wildes, R.P.: Spatiotemporal multiplier networks
  for video action recognition. In: CVPR (2017)

\bibitem{feichtenhofer2016convolutional}
Feichtenhofer, C., Pinz, A., Zisserman, A.: Convolutional two-stream network
  fusion for video action recognition. In: CVPR (2016)

\bibitem{fernando2017going}
Fernando, T., Denman, S., Sridharan, S., Fookes, C.: Going deeper: Autonomous
  steering with neural memory networks. In: CVPR (2017)

\bibitem{gaidon2016virtual}
Gaidon, A., Wang, Q., Cabon, Y., Vig, E.: Virtual worlds as proxy for
  multi-object tracking analysis. In: CVPR (2016)

\bibitem{ganin2015unsupervised}
Ganin, Y., Lempitsky, V.: Unsupervised domain adaptation by backpropagation.
  In: ICML (2015)

\bibitem{huang2016densely}
Huang, G., Liu, Z., Weinberger, K.Q., van~der Maaten, L.: Densely connected
  convolutional networks. arXiv preprint arXiv:1608.06993  (2016)

\bibitem{jain2015car}
Jain, A., Koppula, H.S., Raghavan, B., Soh, S., Saxena, A.: Car that knows
  before you do: Anticipating maneuvers via learning temporal driving models.
  In: IV (2015)

\bibitem{jain2016brain4cars}
Jain, A., Koppula, H.S., Soh, S., Raghavan, B., Singh, A., Saxena, A.:
  Brain4cars: Car that knows before you do via sensory-fusion deep learning
  architecture. arXiv preprint arXiv:1601.00740  (2016)

\bibitem{jain2016recurrent}
Jain, A., Singh, A., Koppula, H.S., Soh, S., Saxena, A.: Recurrent neural
  networks for driver activity anticipation via sensory-fusion architecture.
  In: ICRA (2016)

\bibitem{JhuangICCV2013}
Jhuang, H., Gall, J., Zuffi, S., Schmid, C., Black, M.J.: Towards understanding
  action recognition. In: ICCV (2013)

\bibitem{klingelschmitt2016probabilistic}
Klingelschmitt, S., Damerow, F., Willert, V., Eggert, J.: Probabilistic
  situation assessment framework for multiple, interacting traffic participants
  in generic traffic scenes. In: IV (2016)

\bibitem{kooij2014context}
Kooij, J.F.P., Schneider, N., Flohr, F., Gavrila, D.M.: Context-based
  pedestrian path prediction. In: ECCV (2014)

\bibitem{ped_benchmark}
Kooij, J.F.P., Schneider, N., Flohr, F., Gavrila, D.M.: Context-based
  pedestrian path prediction. In: ECCV (2014)

\bibitem{koppula2016anticipating}
Koppula, H.S., Saxena, A.: Anticipating human activities using object
  affordances for reactive robotic response. TPAMI  (2016)

\bibitem{li2017unified}
Li, X., Li, L., Flohr, F., Wang, J., Xiong, H., Bernhard, M., Pan, S., Gavrila,
  D.M., Li, K.: A unified framework for concurrent pedestrian and cyclist
  detection. T-ITS  (2017)

\bibitem{liebner2013generic}
Liebner, M., Ruhhammer, C., Klanner, F., Stiller, C.: Generic driver intent
  inference based on parametric models. In: ITSC (2013)

\bibitem{ma2016learning}
Ma, S., Sigal, L., Sclaroff, S.: Learning activity progression in lstms for
  activity detection and early detection. In: CVPR (2016)

\bibitem{morris2011lane}
Morris, B., Doshi, A., Trivedi, M.: Lane change intent prediction for driver
  assistance: On-road design and evaluation. In: IV (2011)

\bibitem{ohn2014head}
Ohn-Bar, E., Martin, S., Tawari, A., Trivedi, M.M.: Head, eye, and hand
  patterns for driver activity recognition. In: ICPR (2014)

\bibitem{olabiyi2017driver}
Olabiyi, O., Martinson, E., Chintalapudi, V., Guo, R.: Driver action prediction
  using deep (bidirectional) recurrent neural network. arXiv preprint
  arXiv:1706.02257  (2017)

\bibitem{pentland1999modeling}
Pentland, A., Liu, A.: Modeling and prediction of human behavior. Neural
  computation  (1999)

\bibitem{pool2017using}
Pool, E.A., Kooij, J.F., Gavrila, D.M.: Using road topology to improve cyclist
  path prediction. In: IV (2017)

\bibitem{ramanathan2016detecting}
Ramanathan, V., Huang, J., Abu-El-Haija, S., Gorban, A., Murphy, K., Fei-Fei,
  L.: Detecting events and key actors in multi-person videos. In: CVPR (2016)

\bibitem{rasouli2017agreeing}
Rasouli, A., Kotseruba, I., Tsotsos, J.K.: Agreeing to cross: How drivers and
  pedestrians communicate. arXiv preprint arXiv:1702.03555  (2017)

\bibitem{richterplaying}
Richter, S.R., Hayder, Z., Koltun, V.: Playing for benchmarks. In: ICCV (2017)

\bibitem{richter2016playing}
Richter, S.R., Vineet, V., Roth, S., Koltun, V.: Playing for data: Ground truth
  from computer games. In: ECCV (2016)

\bibitem{GTAgame}
Rockstar-Games: Grand Theft Auto V: PC single-player mods (2018),
  \url{http://tinyurl.com/yc8kq7vn}

\bibitem{GTA_file}
Rockstar-Games: Policy on posting copyrighted Rockstar Games material (2018),
  \url{http://tinyurl.com/yc8kq7vn}

\bibitem{ros2017semantic}
Ros, G., Sellart, L., Villalonga, G., Maidanik, E., Molero, F., Garcia, M.,
  Cede{\~n}o, A., Perez, F., Ramirez, D., Escobar, E., et~al.: Semantic
  segmentation of urban scenes via domain adaptation of synthia. In: DACVA
  (2017)

\bibitem{ryoo2011human}
Ryoo, M.S.: Human activity prediction: Early recognition of ongoing activities
  from streaming videos. In: ICCV (2011)

\bibitem{ryoo2009spatio}
Ryoo, M.S., Aggarwal, J.K.: Spatio-temporal relationship match: Video structure
  comparison for recognition of complex human activities. In: ICCV (2009)

\bibitem{schulz2015controlled}
Schulz, A.T., Stiefelhagen, R.: A controlled interactive multiple model filter
  for combined pedestrian intention recognition and path prediction. In: ITSC
  (2015)

\bibitem{smith2007overview}
Smith, R.: An overview of the tesseract ocr engine. In: ICDAR. IEEE (2007)

\bibitem{soomro2016online}
Soomro, K., Idrees, H., Shah, M.: Online localization and prediction of actions
  and interactions. arXiv preprint arXiv:1612.01194  (2016)

\bibitem{soomro2016predicting}
Soomro, K., Idrees, H., Shah, M.: Predicting the where and what of actors and
  actions through online action localization. In: CVPR (2016)

\bibitem{soomro2012ucf101}
Soomro, K., Zamir, A.R., Shah, M.: Ucf101: A dataset of 101 human actions
  classes from videos in the wild. arXiv preprint arXiv:1212.0402  (2012)

\bibitem{tawari2014looking}
Tawari, A., Sivaraman, S., Trivedi, M.M., Shannon, T., Tippelhofer, M.:
  Looking-in and looking-out vision for urban intelligent assistance:
  Estimation of driver attentive state and dynamic surround for safe merging
  and braking. In: IV (2014)

\bibitem{volvoaccident}
Volvo: Volvo trucks safety report 2017. Tech. rep., Volvo Group (2017)

\bibitem{vondrick2016anticipating}
Vondrick, C., Pirsiavash, H., Torralba, A.: Anticipating visual representations
  from unlabeled video. In: CVPR (2016)

\bibitem{TSN}
Wang, L., Xiong, Y., Wang, Z., Qiao, Y., Lin, D., Tang, X., Van~Gool, L.:
  Temporal segment networks: towards good practices for deep action
  recognition. In: ECCV (2016)

\bibitem{wang2017hierarchical}
Wang, X., Ji, Q.: Hierarchical context modeling for video event recognition.
  TPAMI  (2017)

\bibitem{zyner2017long}
Zyner, A., Worrall, S., Ward, J., Nebot, E.: Long short term memory for driver
  intent prediction. In: IV (2017)

\end{thebibliography}

